Exploring the Use of Attention within an Neural Machine Translation Decoder States to Translate Idioms

Idioms pose problems to almost all Machine Translation systems. This type of language is very frequent in day-to-day language use and cannot be simply ignored. The recent interest in memory augmented models in the field of Language Modelling has aided the systems to achieve good results by bridging long-distance dependencies. In this paper we explore the use of such techniques into a Neural Machine Translation system to help in translation of idiomatic language.

==> sections/analysis-old.tex <==
In this section we will analyse the behaviour of the \attentivenmt models. We split the analysis into a section about the behaviour on regular language (\mysec \ref{sub:regular}) and a section about the  behaviour on idiomatic language (\mysec \ref{sub:idioms}). We provide a discussion on our findings in \mysec \ref{sub:discussion}.

\subsection{Regular Language}
\label{sub:regular}

The first line of Figure \ref{fig:bleu} shows a plot of the BLEU scores obtained by the systems for different sentence lengths over the \wmtfour and \wmtfive test corpora in the \deen direction. Once again the SMT systems achieve a superior performance over longer sentences, although for this language pair it was the best system among all different lengths. The NMT baseline performed the second best in both test corpora and we can see from the figure that the performance starts to degrade on sentences longer than 40 words in the case of \wmtfour and as soon as 20 words on the \wmtfive.

Despite the fact that both of our \attentivenmt with \textit{dot} encoder content functions maintained a similar performance among sentences up to 50 words in length, the performance degrades as the sentence length is beyond the length used in training. In addition, although that performance kept almost constant, it was far below the baselines. On the \wmtfive data, the performance of our models degraded as soon as we move to sentences longer than 10 words.

\begin{figure*}[tb]
  \centering
  % first line
  \begin{subfigure}[b]{0.45\textwidth}
     \includegraphics[width=\linewidth]{images/bleu/bleu_de-en_wmt2014.pdf}
     \caption{\wmtfour}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
     \includegraphics[width=\linewidth]{images/bleu/bleu_de-en_wmt2015.pdf}
     \caption{\wmtfive}
  \end{subfigure}
  \caption{BLEU scores (DE/EN)}
  % second line
  \begin{subfigure}[b]{0.45\textwidth}
     \includegraphics[width=\linewidth]{images/bleu/bleu_en-de_wmt2014.pdf}
     \caption{\wmtfour}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
     \includegraphics[width=\linewidth]{images/bleu/bleu_en-de_wmt2015.pdf}
     \caption{\wmtfive}
  \end{subfigure}
  \caption{BLEU scores (EN/DE)}
  % third line
  \begin{subfigure}[b]{0.45\textwidth}
     \includegraphics[width=\linewidth]{images/bleu/bleu_de-en_idioms.pdf}
     \caption{(DE/EN)}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\textwidth}
     \includegraphics[width=\linewidth]{images/bleu/bleu_en-de_idioms.pdf}
     \caption{(EN/DE)}
  \end{subfigure}
  \caption{BLEU scores on idioms corpus}
  \label{fig:bleu}
\end{figure*}

In the middle row of Figure \ref{fig:bleu} we show the BLEU scores obtained over the \wmtfour and \wmtfive corpora for all the systems in the \enge direction. In these results, we can see from the figure that the \attentivenmt with \singscore and \textit{dot} encoder content function perform better than all the baselines for sentences up to 40 words in the \wmtfour corpus and up to 30 words in \wmtfive corpus. Although the SMT model outperforms our \attentivenmt models on sentences longer than 50 words in \wmtfour corpus, the difference is not as large as in the other experiments. In addition, Dot \& \attentivenmt with \singscore was the best system for sentences up to 30 words in length but its performance degraded fast once the sentence length was increased to beyond 60 words in length. Although the General \& \attentivenmt performed slightly below the other \attentivenmt for shorter sentences, it performed better on longer sentences, although its performance started to degrade when the sentence of the length was 60 words or larger. Interestingly, the SMT baseline achieved larger BLEU scores for  sentences between 40 and 60 words long, but its performance dropped below our best \attentivenmt and the NMT baseline.

\subsection{Idiomatic Language}
\label{sub:idioms}

Having analysed the performance of the systems over the test corpora containing regular language, we now provide an analysis over the idioms corpora used in the experiment. In the bottom row of Figure \ref{fig:bleu} show the performance of the systems for the \deen language pair tested over the corpus of idioms of \newcite{fritzinger:2010} in both directions. Once again, we display the BLEU scores obtained by the our and the baseline systems over sentences of different lengths.

It is interesting to observe how a similar pattern of performance occurs in the DE/EN direction. All the systems improve their performance as the length of sentences increased up to 40 words and, in addition, all the systems also had a degradation in performance once the sentence length went beyond 40 words. In addition, the SMT system, although the best system overall for this task, had the worst performance on the longest sentences of 80 words.

In the EN/DE direction, both the \attentivenmt had a superior performance on sentences up to 40 words in length. Once past that sentence length, there is a rapid degradation in the performance of both \attentivenmt systems although the SMT and NMT baselines increased their performance on the longer sentences. In addition, it is important to note that the lengths of the idiomatic sentences in the English input are in general shorter than their German counterparts after tokenization.

\subsection{Discussion}
\label{sub:discussion}

The results obtained by our \attentivenmt are mixed. Nevertheless, our \attentivenmt is on par with strong baselines composed of single models, including the state-of-the-art NMT model for the \deen language pair. In fact, our models consistently perform better than those NMT models in almost every sentence length in both directions analysed in terms of BLEU scores. The \attentivenmt, in general, perform well on sentences up to 50 words of length but its performance degrades very rapidly once that threshold is surpassed. The only exception to this behaviour is the \deen direction in which the \attentivenmt systems do not perform well on any sentence length.

An import point of consideration is that, as shown by \newcite{jean-wmt:2015}, NMT models often struggle when translating into English (in comparison to translating into other languages) and even the inclusion of an attention module to score past states of the decoder seems to work only in limited cases.

When translating different languages, there are interactions between input and output words that are highly informative to the system when making the next prediction and that are captured via word alignments \cite{koehn:2010}. By introducing a module to score states of the decoder and subsequently merge this information to the alignments calculated by the attention module over the encoder states (as we do in Eq. \ref{eq:concat_attentive_nmt}) we are introducing a bias towards the decoder states and, thus, we may be weakening the information carried about input/output alignments. If the model is not robust enough to balance this trade off, it will fail and produce poor translations, a fact that is observed in several of our models. For example, all of our \attentivenmt models with a \emph{general} encoder content function failed to converge for the \deen language pair in all experiments and most of our systems failed to achieve the same level of performance as the baselines.

Nevertheless, although we recognize the introduction of the bias, we also show that the \attentivenmt models improved the translations from \en into \de, including the translation of idioms. Given the fact that the \de language has long-distance dependencies in its syntax, this result may be an indication that our model helps in bridging those dependencies by bringing forward past information that may have faded from context at the target side with the \textit{smoothing effect} as shown in the language modeling experiments of \newcite{salton:2017b}. However, that improvement is not observed when \en is the target side, which also indicates that the introduced bias can hurt the performance of the models.

